Learning Hierarchical Control for Robust In-Hand Manipulation

Robotic in-hand manipulation has been a long-standing challenge due to the complexity of modelling hand and object in contact and of coordinating finger motion for complex manipulation sequences. To address these challenges, the majority of prior work has either focused on model-based, low-level controllers or on model-free deep reinforcement learning that each have their own limitations. We propose a hierarchical method that relies on traditional, model-based controllers on the low-level and learned policies on the mid-level. The low-level controllers can robustly execute different manipulation primitives (reposing, sliding, flipping). The mid-level policy orchestrates these primitives. We extensively evaluate our approach in simulation with a 3-fingered hand that controls three degrees of freedom of elongated objects. We show that our approach can move objects between almost all the possible poses in the workspace while keeping them firmly grasped. We also show that our approach is robust to inaccuracies in the object models and to observation noise. Finally, we show how our approach generalizes to objects of other shapes.

==> text/4_dataset.tex <==
\section{Data Collection} \label{chpt:DataCollection}
% \jean{tooooo long. Much of this can go to appendix.}
% \wenzhen{Done}
% What we are doing. Why we do it. 
For the purpose of training and testing our method, we collect a comprehensive dataset of the object's initial poses $\boldsymbol{X}_0$ and goal poses $\boldsymbol{X}_g$ which are all reachable. Details of the sampling method is introduced in Appendix \ref{append:dataset}.
% We conduct the data collection based on a systematic analysis of the manipulation states, based on both the object pose $\boldsymbol{X}$ and contact configuration $\boldsymbol{C}$. 
% \begin{figure}[h]
%     \centering
%     \small
%     \includegraphics[width=1\textwidth]{./figure/PoseSpace3.png}
%     \vspace{-5pt}
%     \caption{\jean{I really like this figure and I think it should come much earlier to visualize the overall idea of the necessity of switching between different behaviours.} \jean{I would not use the stripy stuff for the inner ellipses. Just use solid colours with some transparency. Then the C's are easier to read. Also for (b), can we have less numbers at the ticks especially on the y-axis? But x-axis would benefit too. } (a) A schematic of the object pose space, and the relationship between different contact configuration $\boldsymbol{C}$s and grasp posture $\mathbb{F}$s. Each $\boldsymbol{C}$ covers a range of $\boldsymbol{X}$s, that the hand can transfer between them via reposing, and different $\boldsymbol{C}$s may have some overlapping areas, that the state can transfer between them using sliding or flipping. 
%     (b) Examples of the range of different $\boldsymbol{C}$s on the object pose space.
%     \wenzhen{TODO: Update the F2 F3 examples}
%     } 
%     \vspace{-15pt}
%     \label{fig:goal_vis}
% \end{figure}
% \jean{This part is still important in the main paper.}
%\struct{How we devide things into easy, med, and hard groups, and why we do it.}
We further divide the dataset of $\boldsymbol{X}_0$ and $\boldsymbol{X}_g$ pairs into three groups: Easy Goal, Medium Goal and Hard Goal. In the Easy Goal group, $\boldsymbol{X}_0$ and $\boldsymbol{X}_g$ are in the range of same $\boldsymbol{C}$, so the robot could reach the goal using only reposing. The Medium Goal group contains pairs that $\boldsymbol{X}_0$ and $\boldsymbol{X}_g$ are in the same $\mathbb{F}$, so that sliding might be required to transfer to a different $\boldsymbol{C}$. The Hard Goal group includes pairs of arbitrary $\boldsymbol{X}_0$s and $\boldsymbol{X}_g$s, so that flipping is necessary if $\boldsymbol{X}_0$ and $\boldsymbol{X}_g$ are in different $\mathbb{F}$s. 
% The average distances between $\boldsymbol{X}_0$s and $\boldsymbol{X}_g$s are reported in Table~\ref{tab:GoalGroups}.


